Layer-Dependent Charge State Lifetime of Single Se Vacancies in WSe$_2$

Defect engineering in two-dimensional semiconductors has been exploited to tune the optoelectronic properties and introduce new quantum states in the band gap. Chalcogen vacancies in transition metal dichalcogenides in particular have been found to strongly impact charge carrier concentration and mobility in 2D transistors as well as feature sub-gap emission and single-photon response. In this letter, we investigate the layer-dependent charge state lifetime of Se vacancies in WSe$_2$. In one monolayer WSe$_2$, we observe ultrafast charge transfer from the lowest unoccupied orbital of the top Se vacancy to the graphene substrate within (1.0 $\pm$ 0.2) ps measured via the current saturation in scanning tunneling approach curves. For Se vacancies decoupled by TMD multilayers, we find a sub-exponential increase of the charge lifetime from (62 $\pm$ 14) ps in bilayer to few nanoseconds in four-layer WSe$_2$, alongside a reduction of the defect state binding energy. Additionally, we attribute the continuous suppression and energy shift of the dI/dV in-gap defect state resonances at very close tip--sample distances to a current saturation effect. Our results provide a key measure of the layer-dependent charge transfer rate of chalcogen vacancies in TMDs.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
